GenPlanX. Generation of Plans and Execution

Classical AI Planning techniques generate sequences of actions for complex tasks. However, they lack the ability to understand planning tasks when provided using natural language. The advent of Large Language Models (LLMs) has introduced novel capabilities in human-computer interaction. In the context of planning tasks, LLMs have shown to be particularly good in interpreting human intents among other uses. This paper introduces GenPlanX that integrates LLMs for natural language-based description of planning tasks, with a classical AI planning engine, alongside an execution and monitoring framework. We demonstrate the efficacy of GenPlanX in assisting users with office-related tasks, highlighting its potential to streamline workflows and enhance productivity through seamless human-AI collaboration.

==> extras.tex <==

%\sunandita{The AgentSpace framework built by Google for banking. However, they don't have any paper.}

%\daniel{I have seen that most of these types are self-explanatory. So, sorry, but let us keep them unexplained. We can always rethink this decision}
% just a first draft of the high level description
%The types under \texttt{graph} relate to graphics that can be added to slides or other containers. \texttt{data-type} relates to different ways to structure information on datasets.  \texttt{email} types represent. The \texttt{agent} types represent the entities that interact with the system. Human agents are users, while AI agents are automated processes that assist in task execution. 
%%
%The \texttt{data-file} types are used for storing structured data in excel and csv formats, enabling easy data manipulation and sharing. The \texttt{data} types represent various forms of data and content: dataframes are structured datatables, text is unstructured data, graphs are visual representations, and titles provide descriptive labels.
%%
%The \texttt{file} types, comprising \texttt{api}, \texttt{data-file}, \texttt{pdf-file}, \texttt{word-file}, \texttt{text-file}, and \texttt{powerpoint-file}, cover a range of file formats used for data exchange, documentation, and presentation. The \texttt{contents} types represent various elements and entities within the system that are manipulated or generated during task execution.
%%
%Finally, the \texttt{object} types are categories that help organize and manage the different components and interactions within the domain.
%These types allow for a wide range of operations and interactions within the domain.

%%


\alberto{Since the new action is very simple, I feel the current section is too short and does not add much value. Thoughts?}

%%This action adds a graph to a slide within a presentation. The precondition of action specifies the conditions that must be met before the action can be executed. In the case of the {\tt add-to-slide} action, these conditions are: the slide \texttt{?s} must be available, meaning it has been created by a previous action; the graph \texttt{?g} must be available, indicating that it has also been created; the slide \texttt{?s} must be part of the presentation \texttt{?p}, ensuring that the slide is correctly associated with the intended presentation; and the presentation \texttt{?p} must be available, meaning it has been created. %Add the agent here

%%The \texttt{add-to-slide} action involves the following effects: once the graph \texttt{?g} is added to the slide, it is no longer available for further use, indicating that it has been allocated to a specific slide; the slide \texttt{?s} becomes unavailable after the graph is added, suggesting that each slide can only contain one graph at a time; the graph \texttt{?g} is now part of the slide \texttt{?s}, establishing the relationship between the graph and the slide; and the action incurs a cost, represented by an increase in the \texttt{total-cost} metric by 1. %This could be used to track resource usage or effort involved in adding the graph to the slide.

%%The type \texttt{graph} in this domain can represent multiple specific types of graphs, such as \texttt{pie-chart}, \texttt{bar-chart}, or \texttt{histogram}. This flexibility allows the action to be applicable to various kinds of graphical data representations, making it versatile for different presentation needs. The action is designed to ensure that each slide can only contain one graph, maintaining a clear and organized structure within the presentation.
%The rest of the actions defined in this domain can be found in the Appendix.
% Removed comment from action
%\daniel{enumerate all actions or add it to the Appendix}
%\daniel{this is something we might want to discuss}


% \ram{We need to generalize the prompt generation to be dynamic atleast in theory, and say that it is currently static. Model Context Protocol(MCP) has become the standard for agents to know what tools and actions are possible and this can be configured. Similarly, I think we should say "or MCP can be leveraged to dynamically populate this information". This applies to some of the prompt sections. Let's decide to make this point or ignore this quickly. }




Each component of the prompt is included to facilitate a structured and efficient response process. The generic task definition provides clarity and focus, while the domain types and predicates offer a framework for data representation. Constraints on the output ensure consistency, and the set of intents aids in categorizing and addressing queries. Finally, the database schemas provide the necessary data context for generating accurate responses. 

By incorporating these components, the prompt ensures a comprehensive and systematic approach to handling banking-related queries, leveraging structured data and predefined guidelines to generate accurate and relevant responses.


%, which are structured as follows: %has the following objects
%\daniel{the intention is good, but too sparse. we have a better more compressed way to show it. Also, take into account that object is the top level of the hierarchy. Also, there is no type called types. That is a keyword to define them in PDDL}
\iffalse
\dirtree{%
.1 types.
.2 graph.
.3 pie-chart.
.3 bar-chart.
.3 histogram.
.2 data-type.
.3 column.
.3 value-counts.
.3 count.
.2 email.
.3 input-email.
.3 output-email.
.2 agent.
.3 human-agent.
.3 ai-agent.
.2 data-file.
.3 excel-file.
.3 csv-file.
.2 data.
.3 dataframe.
.3 text.
.3 graph.
.3 title.
.2 file.
.3 api.
.3 data-file.
.3 pdf-file.
.3 word-file.
.3 text-file.
.3 powerpoint-file.
.2 contents.
.3 row.
.3 file.
.3 email.
.3 data.
.3 model.
.3 data-contents.
.3 response.
.3 query.
.3 chat-history.
.3 ml-algorithm.
.3 presentation.
.3 appointments.
.3 appointments-item.
.3 slide.
.2 object.
.3 contents.
.3 data-type.
.3 agent.
.3 language.
.3 session.
}
\bigskip
\fi


 such as: 
      \begin{itemize}
          \item \textbf{graph:} 'pie-chart', 'bar-chart', 'histogram'
          \item \textbf{data-type:} 'column', 'value-counts', 'count'
          \item \textbf{email:} 'input-email', 'output-email'
          \item \textbf{agent:} 'human-agent', 'ai-agent'
          \item \textbf{data-file:} 'excel-file', 'csv-file'
          \item \textbf{data:} 'dataframe', 'text', 'graph', 'title'
          \item \textbf{file:} 'api', 'data-file', 'pdf-file', 'word-file', 'text-file', 'powerpoint-file'
          \item \textbf{contents:} 'row', 'file', 'email', 'data', 'model', 'data-contents', 'response', 'query', 'chat-history', 'ml-algorithm', 'presentation', 'appointments', 'appointments-item', 'slide'
          \item \textbf{object:} 'contents', 'data-type', 'agent', 'language', 'session'
      \end{itemize}

\begin{table}[ht!]
\centering
\footnotesize
\begin{tabular}{|>{\ttfamily}l|>{\ttfamily}l|}
  \hline
  \textbf{Predicate}  & \textbf{Arguments} \\ \hline
  in                  & ?c -- contents, \quad ?c1 -- contents \\ \hline
  in-data             & ?dt -- data-type, \quad ?d -- contents \\ \hline
  in-graph            & ?c -- contents, \quad ?c1 -- contents, \quad ?c3 -- graph \\ \hline
  available           & ?o -- object \\ \hline
  used                & ?c -- contents \\ \hline
  data-type-contents  & ?dt -- data-type, \quad ?dc -- data-contents \\ \hline
  web-search-result   & ?q -- text, \quad ?r -- text \\ \hline
  deep-research-result& ?q -- text, \quad ?r -- text \\ \hline
  merged-answer       & ?q -- text, \quad ?r -- text \\ \hline
  last-result         & ?q -- text, \quad ?l -- text \\ \hline
  query-result        & ?d -- dataframe, \quad ?q -- query, \quad ?d1 -- data \\ \hline
  answer-llm          & ?q -- text, \quad ?r -- text \\ \hline
  extract-result      & ?a -- api, \quad ?c -- column, \quad ?v -- text, \quad ?d -- data \\ \hline
  done-merge          & (none) \\ \hline
  reference           & ?c -- column, \quad ?d -- dataframe \\ \hline
  done-query          & ?q -- query \\ \hline
  done-question       & ?q -- text \\ \hline
  modified            & ?d -- dataframe, \quad ?c -- contents, \quad ?co -- column, \quad ?t -- text, \quad ?d1 -- dataframe \\ \hline
  added-value         & ?d -- dataframe, \quad ?c -- contents, \quad ?co -- column, \quad ?t -- text, \quad ?d1 -- dataframe \\ \hline
  merged              & ?d -- dataframe, \quad ?d1 -- dataframe, \quad ?d2 -- dataframe \\ \hline
  deleted             & ?d -- dataframe, \quad ?d1 -- dataframe, \quad ?d2 -- dataframe \\ \hline
  sent-contents       & ?rc -- contents, \quad ?r -- response \\ \hline
  sent                & ?r -- response \\ \hline
  sent-email          & ?e -- output-email, \quad ?c -- contents \\ \hline
  read-email-contents & ?c -- contents, \quad ?f -- file, \quad ?e -- input-email \\ \hline
  replied-email       & ?e -- input-email \\ \hline
  email-read          & ?e -- input-email \\ \hline
  email-parsed        & ?e -- input-email \\ \hline
  notified            & ?e -- output-email, \quad ?c -- contents \\ \hline
  explained           & ?c -- contents, \quad ?c1 -- contents \\ \hline
  translated          & ?c -- contents, \quad ?l -- language, \quad ?c1 -- contents \\ \hline
  summarized          & ?c -- contents, \quad ?c1 -- contents \\ \hline
  search-result       & ?t -- text, \quad ?q -- text, \quad ?t1 -- text \\ \hline
  info-on             & ?d -- data-contents, \quad ?g -- graph, \quad ?p -- presentation \\ \hline
  appointments-read   & ?s -- appointments \\ \hline
  appointments-contents & ?s -- appointments, \quad ?d -- dataframe \\ \hline
  learned-model       & ?m -- model, \quad ?d -- dataframe, \quad ?c -- column \\ \hline
  matched             & ?f1 -- file, \quad ?f2 -- file, \quad ?f3 -- file, \quad ?m -- dataframe \\ \hline
\end{tabular}
\caption{List of pre-defined predicates}
\label{tab:predicates}
\end{table}



%Alfredo: update the bellow with the running example

% As an example, given the request {\it Read genplanx/annual-report.csv and generate a bar chart from 'balance' against reference column 'year'. Create a slide with the bar chart titled 'Balance over years', and add it to a presentation. Save the presentation in the file genplanx/graph.pptx}, the LLM could return the dictionary in Figure~\ref{fig:output-dict}.

% The dictionary in Figure~\ref{fig:output-dict} represents the output of the LLM tasked with generating a presentation based on specific data inputs. Each key-value pair in the dictionary corresponds to an object of the task, such as presentations, slides, titles, and data files. The \texttt{init\_state} and \texttt{goals} keys define the initial and desired states of the task, respectively.

% \begin{itemize}
%     \item \textbf{Presentation and Slides}: The dictionary includes entries for a presentation and its associated slides, each identified by a unique key (e.g., \texttt{presentation1}, \texttt{slide1}).
%     \item \textbf{Titles and Texts}: Titles and text elements are included to provide context and content for the slides.
%     \item \textbf{Data Files and Queries}: Data files and queries are specified to extract and manipulate data needed for the presentation.
%     \item \textbf{State Representation}: The \texttt{init\_state} describes the initial conditions, such as the presence of text in a PDF file or the availability of query results. The \texttt{goals} outline the desired outcomes, such as the inclusion of text in slides and the completion of queries.
% \end{itemize}

% This structured approach ensures that the language model can effectively interpret and respond to complex queries by leveraging predefined guidelines and structured data.


%The Execution component receives this high-level plan and translate it into the low-level actions (code) that will be executed into the real-world.
%%
%The Execution module will periodically sense the real-world and translate the low-level observations into high-level symbols in PDDL.

%This information is sent to the Monitoring module, which will check whether the plan is going as expected or the execution/real-world have deviated from the planned behavior.
%%
%When this occurs, Monitoring incorporates three different modules capable of addressing these scenarios.
%%
%Replanning is able to detect failures in the execution and generates a new plan to achieve the original goal~\cite{lpgfoxetal06},  or even change the goal~\cite{ecai23-replanning}.
%%
%The Goal Reasoning module can also change the goals through detecting opportunities when the environment/real-world changes~\cite{icaps21-opportunities}, or by analyzing the structure of the goals~\cite{icaps24-symbolic-centroids}.
%%
%Finally, the Learning module stores the interactions of the planning agent with the real-world in order to learn the action costs~\cite{morales2024learning} or predict the appearance of new goals~\cite{aicomm18-learning,aicomm18-anticipatory}.

%\daniel{this is not exactly the architecture. Right now, there is no learning, nor goal reasoning. Replanning sould not be part of monitoring, but a call to the planner. Probably, we can remove this figure and just leave the one at the beginning.}




% \begin{figure}[hbt]
%     \centering
%     \includegraphics[width=\textwidth]{example-pptx}
%     \caption{Example of request and plan generated and executed.}
%     \label{fig:example-pptx}
% \end{figure}



% Arguably less relevant \daniel{Natural language and planning. Early work on parsing WikiHow and extracting the objects, actions and plans~\cite{dart2010}. Also some work from Lindsay, narrative generation by Patrick Hasslum}

% Done \daniel{I think we can start with a subsection on LLM planning (CoT, React and others), and then a second subsection that starts with the critiques (Raos papers). And then talks about hybrid approaches. Finally, a third section could talk about office-related planning tasks. We can mention softbots, but also work on planning + workflows - you can see my paper on that. Please rewrite if you agree} 

Intent: What services do you offer?
Output:
{"chat-response": {"type": "response", "value": "We offer a variety of services including personal banking, loans, and investment advice."}, "init_state": {"type": "state", "value": "(available chat-response)"}, "goals": {"type": "state", "value": "(and (sent chat-response))"}}


%More specifically, as we may see in Listing~\ref{lst:read-data-python}, it extracts the slide and graph object from the state using the appropriate parameters from the list in the input. Then, depending on the graph type, it adds the correct one to the slide. Finally, after updating the state with the new slide, it returns it. This change to the execution state may cause a consequent change to the PDDL state (the one we plan on).

%\daniel{talk about action\_success. Signature common to all those actions. Example. Right now, monitoring only happens through this low-level actions. There is no return from low-level state to high-level state as in other architectures. Mention PELEA. Instead all the monitoring works happens with the \_success actions. Talk about when these actions return new goals in the execution state. Provide an example.}

% \begin{figure}[hbt]
%     \centering
%     \includegraphics[width=0.7\linewidth]{example/plan_execution_for_operating_on_appointments_part1.PNG}
%     \caption{Performing operations on the retrieved appointments.}
%     \label{fig:enter-label1}
% \end{figure}

%The RAE+UPOM system~\cite{patra2021deliberative} does integration of planning and execution using operational models. Operational models are programs that describe {\em how} actions are performed. RAE is the acting engine which takes advice from the planner UPOM. UPOM performs UCT-like search by doing simulated rollouts of the operational models to recommend the best course of action. Unlike us, RAE+UPOM does support problem specification in natural language. RAE+UPOM has been evaluated on some simulated domains~\cite{patra2021deliberative} and a real world software defined network domain~\cite{patra2021using}.


        % init\_state & State & \texttt{(in dataframe1 data-file1) (available query1) (query-result dataframe1 query1 filtered-dataframe) (available query2) (query-result dataframe1 query2 reference-dataframe) (reference reference1 reference-dataframe)} \\
        % goals & State & \texttt{(and (done-query query1) (done-query query2) (in-graph filtered-dataframe reference-dataframe bar-chart1) (in bar-chart1 slide1) (in title1 slide1) (in slide1 presentation1) (in presentation1 presentation-file1))} \\

